Predictive Monitoring with Strong Trace Prefixes

Runtime predictive analyses enhance coverage of traditional dynamic analyses based bug detection techniques by identifying a space of feasible reorderings of the observed execution and determining if any of these witnesses the violation of some desired safety property. The most popular approach for modelling the space of feasible reorderings is through Mazurkiewicz's trace equivalence. The simplicity of the framework also gives rise to efficient predictive analyses, and has been the de facto means for obtaining space and time efficient algorithms for monitoring concurrent programs. In this work, we investigate how to enhance the predictive power of trace-based reasoning, while still retaining the algorithmic benefits it offers. Towards this, we extend trace theory by naturally embedding a class of prefixes, which we call strong trace prefixes. We formally characterize strong trace prefixes using an enhanced dependence relation, study its predictive power and establish a tight connection to the previously proposed notion of synchronization preserving correct reorderings developed in the context of data race and deadlock prediction. We then show that despite the enhanced predictive power, strong trace prefixes continue to enjoy the algorithmic benefits of Mazurkiewicz traces in the context of prediction against co-safety properties, and derive new algorithms for synchronization preserving data races and deadlocks with better asymptotic space and time usage. We also show that strong trace prefixes can capture more violations of pattern languages. We implement our proposed algorithms and our evaluation confirms the practical utility of reasoning based on strong prefix traces.

==> Makefile <==
all: Makefile *.tex *.bib
	rm -f *.pyg
	pdflatex -shell-escape --jobname=main main
	bibtex main -min-crossrefs=5
	pdflatex -shell-escape --jobname=main main
	pdflatex -shell-escape --jobname=main main

#	pdflatex -shell-escape --jobname=main "\def\extflag{}\input{main}"
nobib: Makefile *.tex
	rm -f *.pyg
	pdflatex -shell-escape --jobname=main main

quick: Makefile *.tex *.bib
	rm -f *.pyg
	pdflatex -shell-escape --jobname=main main

appendix: Makefile *.tex
	pdflatex -shell-escape --jobname=appendix appendix
#	bibtex main-extended -min-crossrefs=5 
#	pdflatex -shell-escape --jobname=appendix appendix
	pdflatex -shell-escape --jobname=appendix appendix


clean:
	rm -rf *.pyg *.aux *.bbl *.blg *.log *.out *.rel minted-cache main.pdf main.zip	main.fdb_latexmk main.fls appendix.pdf

.PHONY: all clean

zip:
	zip main.zip Makefile *.tex *.bbl mathpartir.sty references.bib frameit.sty llncs.cls fig/*.tex fig/*.pdf tables/*


==> figures/trace-limitation-ww.tex <==
%!TEX root=../main.tex

\begin{figure}[t]
    \centering
    \subfloat[Execution $\tr_5$ \figlabel{ww-race-trace}]{%
        \execution{2}{
            \figev{1}{$\wt(y)$}
            \figev{1}{$\wt(x)$}
            \figev{2}{$\wt(x)$}
            \figev{2}{$\rd(y)$}
        }
    }
    \hfill
    \subfloat[Reordering $\rho_5$ of $\tr_5$ \figlabel{ww-no-race-trace}]{%
        \execution{2}{
            \figev{1}{$\wt(y)$}
            \figev{2}{$\wt(x)$}
            \figev{2}{$\rd(y)$}
        }
    }
    \hfill
    \subfloat[Reordering $\rho'_5$ of $\tr_5$ \figlabel{ww-race-correct-reordering}]{
        \execution{2}{
            \figev{2}{$\wt(x)$}
            \figev{1}{$\wt(y)$}
            \figev{2}{$\rd(y)$}
        }
    }
    % \hfill
    % \subfloat[Reordering $\rho_2$ of $\tr_2$ \figlabel{rwwr-race-correct-reordering}]{
    %     \execution{3}{
    %         \figev{1}{$\wt(y)$}
    %         \figev{3}{$\rd(x)$} 
    %         \figev{2}{$\wt(x)$}
    %         \figev{2}{$\rd(x)$}
    %         \figev{2}{$\rd(y)$}
    %     }
    % }
    \begin{comment}
    \subfloat[Execution $\tr_1$ \figlabel{rwwr-race-trace}]{%
        \smallexecution{3}{
            \smallfigev{1}{$\wt(y)$}
            \smallfigev{1}{$\wt(x)$}
            \smallfigev{1}{$\rd(x)$}
            \smallfigev{3}{$\rd(x)$} 
            \smallfigev{2}{$\wt(x)$}
            \smallfigev{2}{$\rd(x)$}
            \smallfigev{2}{$\rd(y)$}
        }
    }
    \hfill
    \subfloat[Execution $\tr_2$ \figlabel{rwwr-no-race-trace}]{%
        \smallexecution{3}{
            \smallfigev{1}{$\wt(y)$}
            \smallfigev{2}{$\wt(x)$}
            \smallfigev{2}{$\rd(x)$}
            \smallfigev{2}{$\rd(y)$}
        }
    }
    \hfill
    \subfloat[Reordering $\rho_2$ of $\tr_2$ \figlabel{rwwr-race-correct-reordering}]{
        \smallexecution{3}{
            \smallfigev{2}{$\wt(x)$}
            \smallfigev{2}{$\rd(x)$}
            \smallfigev{1}{$\wt(y)$}
            \smallfigev{2}{$\rd(y)$}
        }
    }
    \hfill
    \subfloat[Reordering $\rho_2$ of $\tr_2$ \figlabel{rwwr-race-correct-reordering}]{
        \smallexecution{3}{
            \smallfigev{1}{$\wt(y)$}
            \smallfigev{3}{$\rd(x)$} 
            \smallfigev{2}{$\wt(x)$}
            \smallfigev{2}{$\rd(x)$}
            \smallfigev{2}{$\rd(y)$}
        }
    }
\end{comment}
\caption{Execution $\tr_5$ has a predictable data race $(\ev{t_1}{\wt(y)}, \ev{t_2}{\rd(y)})$, and can not be exposed with trace equivalence. However, it can be exposed by a strong trace prefix $\rho'_5$.}
\figlabel{trace-limitation-ww}
\end{figure}

==> related-work.tex <==
%!TEX root=./main.tex

% \myparagraph{Related Work}{
% Our work is inspired from runtime predictive analysis for testing concurrent programs,
% where the task is to enhance the coverage of naive dynamic analysis techniques to a larger space of correct reorderings~\cite{MaximalCausalModel2013,Said11,RVPredict2014}.
% A key focus here is to improve the scalability of prediction techniques for concurrency bugs such as data races~\cite{cp2012,wcp2017,SHB2018,Pavlogiannis2019,OSR2024,SyncP2021}, deadlocks~\cite{Kalhauge2018,tuncc2023sound}, atomicity violations~\cite{mathur2020atomicity,biswas2014doublechecker,farzan2008monitoring} and more general properties~\cite{huang2015gpredict6,ang2023predictive} for an otherwise intractable problem~\cite{Mathur2020}.
% The theme of our work is to develop efficient algorithms 
% for predictive concurrency bug detection.
% We start with the setting of trace theory~\cite{Mazurkiewicz1987}, where
% questions such as checking whether two events can be flipped,
% which are intractable in general~\cite{grain2024,Mathur2020,kulkarni2021dynamic}, can be answered 
% in constant space.
% More generally, the class of star-connected languages~\cite{Ochmanski85} precisely characterizes those languages that can be monitored efficiently under trace equivalence. 
% The problem of relaxing Mazurkiewicz traces has been studied~\cite{Diekert94}.
% Recent work~\cite{grain2024} has focused on reasoning about commutativity of grains of events. 
% In contrast, our work takes an orthogonal angle and proposes that, for co-safety properties, one might be able to 
% perform relaxations by 
% exploiting semantic properties of programming constructs in multi-threaded shared-memory programs. 
% To this end, we proposed a slightly different formalism where the commutativity between events can be stratified into strong and weak dependencies.
% This simple relaxation allows us to capture a large class of concurrency bugs, while still allowing for some of the algorithmic simplicity that event based commutativity offers.
% }
